Polarization Profiles of Globular Cluster Pulsars from FAST I. 25 Profiles from Previously Known Pulsars

Pulsar polarization profiles are critical for understanding their magnetospheric structures and radiation mechanisms. We present polarization profile measurements for 25 pulsars in globular clusters (GCs) from the observation of the Five-hundred-meter Aperture Spherical radio Telescope (FAST). The diversity of polarization profiles shows complex magnetic structure and emission pattern of pulsars. Among these, the polarization profiles of 15 pulsars were firstly measured. M53A present a 57\% linear polarization ratio, being highest among these 25 GC pulsars. M15H present a 42\% circular polarization ratio, which is the highest among these 25 pulsars. The average ratios of circular and absolute circular polarization of these GC pulsars are -1\% and 10\% respectively, lower than normal pulsars measured with Parkes (\citealt{Oswald2023}), which are 5\% and 32\%, respectively. The Rotation Measure (RM) values of each pulsar were measured, giving the range of pulsar(s) from M3, M5, M15, M71, M53, NGC6517, NGC6539, NGC6760 being 8(1) to 16(1) rad $m^{-2}$, -1(2) to -4(6) rad $m^{-2}$, -70(2) to -76(1) rad $m^{-2}$, -480(14) rad $m^{-2}$ (M71A only), -2(1) rad $m^{-2}$ (M53A only), 187(1) to 212(2) rad $m^{-2}$, 109(1) rad $m^{-2}$ (NGC6539A only), and 102(1) to 129(4) rad $m^{-2}$. The GCs closer to the Galactic plane (GP) tend to have larger RM. This is consistent with previous study (\citealt{Hutschenreuter2022}).

==> readme <==
Dear Colleagues: 

The final publication layout will be produced by using raa.cls. 
Therefore, we strongly encourage you to prepare your LaTeX manuscript 
with this class file. Please unpack raa-package.tar.gz, it includes 

raa.cls        ---- RAA macro class file for LaTeX2e 
sample.tex     ---- a sample file using raa.cls (LaTeX source) 
sample.ps      ---- the PS file created by sample.tex in referee format  
sample.pdf     ---- the PDF file created by sample.tex in referee format  
readme         ---- this file  
f?.eps         ---- three demo figures used in the LaTeX template source
sample2.tex    ---- a sample file for using raa.bst
sample2_fig?.eps -- two demo figures used in sample2.tex
sample2.pdf    ---- the PDF file created by sample.tex in referee format
sample2.bbl    ---- bibliography file using by sample2.tex
bibtex.bib     ---- an example for bibtex file

natbib.sty     ---- This package reimplements the LaTeX \cite command
natnotes.pdf   ---- Brief reference sheet for Natbib (pdf)
raa.bst        ---- Bibliography style file 

Hope you enjoy the use of this macro. Your suggestions and comments are 
highly welcome. Thanks.

Editorial Office
E-mail:  raa@raa-journal.org

